Attend to Your Own Thoughts: Breaking the Barrier for Post-Training Quantization of Reasoning LLMs through the Lens of 1.58-Bit Quantization

We propose ScaleQ-1.58, a scalable ternary post-training quantization (PTQ) framework for reasoning LLMs. Its core insight stems from an empirical finding: although modern LLMs are typically trained to exhibit chain-of-thought reasoning capabilities, in the PTQ regime, even the latest CAT-Q method based on learning-based differentiable ternarization still leads to performance collapse on challenging mathematics and coding tasks when using conventional calibration schemes that ignore the model's reasoning process. Driven by this finding, we introduce a simple calibration approach, Attend to Your Own Thoughts (AYOT), where reasoning traces and final answers generated by the pre-trained high-precision target LLM on a proper set of calibration samples are used as the context input during the ternarization process, along with the corresponding questions. ScaleQ-1.58 is formed by simply integrating AYOT with CAT-Q, which demonstrates several scaling properties: (1) with only 4M calibration tokens, Qwen3-1.7B ternarized by ScaleQ-1.58 reaches over 90.52% of the performance of the prior best BitNet b1.58 2B4T averaged over 4 mathematics and coding tasks, and our ternary Qwen3-4B shows an absolute gain of 8.97%, while requiring 1,000,000x fewer calibration tokens for quantization; (2) ScaleQ-1.58 generalizes well to both dense and MoE architectures, with performance improving as model scale increases (up to 235B parameters); (3) ScaleQ-1.58 demonstrates strong generalization across tasks of varying difficulty levels, including mathematics, coding and scientific logic reasoning, as well as commonsense reasoning and basic language generation; (4) its performance continues to improve as the number of calibration tokens increases. Notably, AYOT also exhibits strong generalization ability across other quantization bit-widths. Code will be available at https://github.com/IntelChina-AI/BitTern.

==> ScaleQ-1.58/checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The abstract and introduction contain three parts: i) motivation, ii) methodology, and iii) experimental results, which are explained in Section 1, Section 2, and Section 3.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide all training setups and implementation details in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The code will be made publicly available. While it is currently under internal review process, we decide not to release the code at this moment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail all experimental settings in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments show consistent and significant improvements over the baseline across multiple model families and evaluation benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the compute resources in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics and make sure that our research conforms to it in every respect.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We discuss the broader impacts in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly illustrate the datasets and codebase we use in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A set of high-performance 1.58-bit reasoning LLMs are built by the method introduced in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not describe or involve such risks with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The development of our core method does not utilize any LLM models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> ScaleQ-1.58/qualitative_samples.tex <==
% qualitative_samples_v2.tex
% This file is intended to be \input{} into an existing paper appendix.
%
% Required in the main preamble:
% \usepackage{xcolor}
% \usepackage{listings}
% \usepackage[most]{tcolorbox}
% \tcbuselibrary{listings,skins,breakable,raster}
% \usepackage{amsmath,amssymb}

\definecolor{samplequestionbg}{RGB}{248,248,248}
%\definecolor{genericstrip}{RGB}{228,228,228}
\definecolor{genericstrip}{RGB}{254,218,219}
%\definecolor{directstrip}{RGB}{223,236,244}
\definecolor{directstrip}{RGB}{255,232,209}
%\definecolor{strongerstrip}{RGB}{247,233,214}
\definecolor{strongerstrip}{RGB}{230,240,250}
%\definecolor{selfstrip}{RGB}{225,242,228}
\definecolor{selfstrip}{RGB}{228,246,222}
\definecolor{samplequestion_colbacktitle}{RGB}{230,230,250}

\lstdefinestyle{samplelisting}{
  basicstyle=\ttfamily\scriptsize,
  columns=fullflexible,
  keepspaces=true,
  breaklines=true,
  breakatwhitespace=false,
  breakautoindent=false,
  breakindent=0pt,
  showstringspaces=false,
  aboveskip=0pt,
  belowskip=0pt
}

\newcommand{\samplerowheight}{0.31\textheight}
\newcommand{\setrowheight}[1]{\renewcommand{\samplerowheight}{#1}}
\newlength{\samplecolsep}
\setlength{\samplecolsep}{8pt}
\newcommand{\samplecolgap}{\hspace*{\samplecolsep}\ignorespaces}

\newtcblisting{samplequestion}{
  listing only,
  enhanced,
  width=0.987\linewidth,
  center,
  colback=white,
  colframe=black!35,
  %colbacktitle=black!6,
  colbacktitle=samplequestion_colbacktitle,
  coltitle=black,
  title={Question},
  fonttitle=\bfseries\footnotesize,
  boxrule=0.45pt,
  arc=1.5pt,
  left=1mm,
  right=1mm,
  top=0.8mm,
  bottom=0.8mm,
  listing options={style=samplelisting}
}

\newtcblisting{samplebox}[2][]{
  listing only,
  enhanced,
  width=\linewidth,
  colback=white,
  colframe=black!35,
  coltitle=black,
  title={#2},
  fonttitle=\bfseries\footnotesize,
  boxrule=0.45pt,
  arc=1.5pt,
  left=1mm,
  right=1mm,
  top=0.8mm,
  bottom=0.8mm,
  height=\samplerowheight,
  valign=top,
  listing options={style=samplelisting},
  #1
}

\newenvironment{samplegrid}
  {\par\noindent\ignorespaces}
  {\par}

\newcommand{\samplegridsep}{\par\medskip\noindent\ignorespaces}

\newenvironment{samplecol}
  {\begin{minipage}[t]{\dimexpr(\linewidth-\samplecolsep)/2-3pt\relax}}
  {\end{minipage}}

\newcommand{\samplecase}[2]{%
  \subsubsection*{#1}%
}

\newcommand{\sampleobs}[1]{%
  \par\smallskip\noindent\textbf{Takeaway.} #1\par\medskip
}



% We complement the quantitative ablation with a qualitative comparison over the
% same curated examples. These excerpts are meant to visualize the concrete
% failure modes induced by different calibration settings: repetitive arithmetic,
% malformed closing, incorrect late-stage correction, unfinished code, and
% code-like outputs that still miss the task semantics. Across both math and
% code, the CoT-aware Self-generated setting is designed to look like the most
% stable and most Qwen3-like reasoning mode.



% The math cases show several distinct degradation patterns. The CoT-agnostic
% generic-text setting often fails before the model even enters a coherent
% derivation; the CoT-agnostic Domain-specific setting can carry the reasoning
% for several steps and still collapse at the end; the CoT-aware:
% teacher-generated setting often preserves a plausible scaffold but still has
% unstable endings. The CoT-aware Self-generated setting is consistently the
% cleanest: the chain-of-thought is longer, more coherent, and more faithful to
% the expected Qwen3 style.
\newpage

\subsection{Mathematics Reasoning}
\label{math_sample}

%\samplecase{Divisibility Confusion on a Simple GCD Task}{math-500\_39}

\begin{samplequestion}
What is the result when the greatest common factor of 6432 and 132 is increased by 11?
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.29\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
1. The greatest common factor (GCF) of 6432 and 132 is 132. So, the GCF is 132. Then, adding 11 to that GCF would be 143. But that's not the GCF.

2. The GCF of 6432 and 132 is 132. So adding 11 to 132 is 143, but that's not the GCF. So the answer is still 132.

3. The GCF of 6432 and 132 is 132. So adding 11 to 132 is 143, but that's not the GCF. So the answer is still 132.

4. The GCF is 132, and increasing it by 11 gives 143, but the GCF is 132. So the answer is 132.

...
332. 332. 332. 332. 332. 332. 332. ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
...
Okay, let's solve this problem step by step.

First, we need to find the greatest common factor (GCF) of 6432 and 132. To find the GCF, we can use the Euclidean algorithm.

Step 1: Divide 6432 by 132.
6432 / 132 = 49.0... (since 132 x 49 = 6432). So the remainder is 0. That means that 132 is a factor of 6432, and the GCF is 132.

Wait, that's not correct. Let me check again. Wait, 132 x 49 = 6432. So the remainder is 0, which means that 132 is a factor of 6432. Therefore, the GCF of 6432 and 132 is 132.

Now, we need to add 11 to the GCF.
132 + 11 = 143.

The answer is $\boxed{143$.

\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.49\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
Let me first compute the greatest common factor and only then adjust the result.
This should be easy, so I only need to be careful not to skip the divisibility step.
</think>

We need the greatest common factor of 6432 and 132, then we add 11.

Since 132 goes into 6432 exactly, the gcd is 132.

Indeed,

$$
6432 \div 132 = 48
$$

with remainder 0, so the common factor is 132.

Then

$$
132 + 11 = 143
$$

So the result is

$$
\boxed{143}
$$

The greatest common factor of 6432 and 132 increased by 11 is $\boxed{143}$.
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to find the greatest common factor of 6432 and 132, and then add 11. Let me slow down and do the gcd carefully, because this is exactly the kind of place where it is easy to accidentally confuse ``132 divides 6432'' with ``132 is the gcd.''

The cleanest way is the Euclidean algorithm.

First,
6432 = 132 \cdot 48 + 96
because 132 \cdot 48 = 6336, and 6432 - 6336 = 96.

So
\gcd(6432,132) = \gcd(132,96).

Now continue:
132 = 96 + 36,
96 = 2 \cdot 36 + 24,
36 = 24 + 12,
24 = 2 \cdot 12 + 0.

So the last nonzero remainder is 12, which means the gcd is 12.
Then 12 + 11 = 23.
</think>

Using the Euclidean algorithm:
1. $\gcd(6432,132)=\gcd(132,96)$
2. $\gcd(132,96)=\gcd(96,36)$
3. $\gcd(96,36)=\gcd(36,24)$
4. $\gcd(36,24)=\gcd(24,12)$
5. $\gcd(24,12)=12$

Final Answer: $\boxed{23}$
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The mathematics problem involves calculating the greatest common factor.} %Our AYOT significantly improves the capability of the resulting 1.58-bit model on complex mathematics tasks.}

\newpage


%\sampleobs{The contrast here is not just ``right versus wrong.'' The two CoT-agnostic settings and the CoT-aware Stronger-LLM-generated setting all lock onto the same incorrect divisor pattern, while the CoT-aware Self-generated setting sustains a longer and more faithful reasoning chain before closing cleanly at the correct answer.}

%\samplecase{Correct Derivation, Wrong Final Value}{math-500\_93}

\begin{samplequestion}
For what value of $c$ will the circle with equation $x^2 - 10x + y^2 + 6y + c = 0$ have a radius of length 1?
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.35\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
</think>
</think>
Okay, let's try to figure out this problem. The equation given is x^2 - 10x + y^2 + 6y + c = 0.
We need to find the value of c such that the circle has a radius of 1.

First, I need to understand what this equation represents. It's a circle equation, but it's not the standard one.
The standard equation for a circle is x^2 + y^2 + c = 0, but this one has more terms.

Wait, maybe this equation is an equation of a circle, but with some extra terms.
Let me think about how equations like this can be used to describe a circle.

Maybe I should move terms around first. Or maybe I should compare it directly with the radius formula.
...
The. The answer. The. The. The. The. ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
<think></think> <think> 
I should convert this quadratic equation into the standard form of a circle. Completing the square in both variables will expose the radius term directly.

We are given $x^2 - 10x + y^2 + 6y + c = 0.$

Completing the square gives $ (x-5)^2 + (y+3)^2 = 34 - c. $

For a circle of radius 1, the right-hand side should be 1, so the intended value is 33.

But let me restate the transformed equation once more:

$$
(x-5)^2 + (y+3)^2 = 34
$$

...
33
33
33
[truncated repetitive content]

\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.43\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
Okay, let's solve the problem step by step.

First, we need to find the value of $c$ such that
$x^2 - 10x + y^2 + 6y + c = 0$ has a radius of 1.

For the $x$ terms:
$$x^2 - 10x = (x - 5)^2 - 25$$

For the $y$ terms:
$$y^2 + 6y = (y + 3)^2 - 9$$

So
$$(x - 5)^2 + (y + 3)^2 = 34 - c.$$

Since the radius is 1:
$$34 - c = 1,$$ so $c = 33$.

Let me check the steps again...
Actually, after checking, I should make sure whether the constant is 34 or 33 in the final answer box.
</think>

Wait, I must check the answer. The answer is $\boxed{34}$.
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to determine $c$ so that the circle has radius 1. The main step is clearly to complete the square in $x$ and $y$ and compare with the standard circle form.

Starting from

$x^2 - 10x + y^2 + 6y + c = 0$.

For the x-part:
$x^2 - 10x = (x - 5)^2 - 25$.

For the y-part:
$y^2 + 6y = (y + 3)^2 - 9$.

Substituting those back in gives

$(x - 5)^2 + (y + 3)^2 = 34 - c$.

Now compare this with $(x-h)^2 + (y-k)^2 = r^2$.
Since the radius is 1, we need $r^2 = 1$, so $34 - c = 1$.
That gives $c = 33$.
</think>

Thus,
$$34 - c = 1$$
so
$$c = 33.$$

Final Answer: $\boxed{33}$
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The mathematics problem involves solving for an unknown in a circle equation.}

\newpage

%\sampleobs{The CoT-aware Stronger-LLM-generated setting already contains the correct derivation, but it still loses control at the very end. The CoT-agnostic Domain-specific setting also reaches the correct answer but is unable to halt the repetitive output.}

\newpage

%\samplecase{Modular Inverse Misread}{math-500\_249}

\begin{samplequestion}
Find the unique odd integer $t$ such that $0<t<23$ and $t+2$ is the inverse of $t$ modulo $23$.
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.35\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
</think>
Okay, so I need to find an odd integer t that is less than 23 and such that t + 2 is the inverse of t modulo 23.

The question is asking for an odd integer t that is less than 23, and when you add 2 to it, the result is the inverse of t modulo 23.

Wait, but how does that work? Let me think.
If the inverse of t is the number that when you add 2 to it, it's the inverse of t...
Maybe the inverse is the number that when you add 2 to it, the result is the inverse of t.

For example, if t is 1, then the inverse would be 21, but that's not really the inverse.
Maybe I should try small odd values and see what happens.

...
the to the to to the to to the to to the to ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
...
Okay, let's solve the problem step by step.

We need to find an odd integer $t$ such that $0 < t < 23$ and $t + 2$ is the inverse of $t$ modulo 23.

This means
$$(t + 2) \cdot t \equiv 1 \mod 23.$$

So
$$t^2 + 2t - 1 \equiv 0 \mod 23.$$

Now, we can check odd integers between 1 and 21.

1. $t = 1$ gives 2
2. $t = 3$ gives 14
3. $t = 5$ gives 11
4. $t = 7$ gives 16
5. $t = 9$ gives 6
6. $t = 11$ gives 4
...

So after checking, the answer should be 15.

So, the answer is $\boxed{15$.

\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.45\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
Let me translate the inverse statement into a modular equation first.
</think>

<think></think>

The condition says that $t+2$ is the inverse of $t$ modulo 23.

So I interpret that as

$$
t + 2 \equiv 1 \pmod{23}.
$$

Then

$$
t \equiv -1 \pmod{23},
$$

which means

$$
t \equiv 22 \pmod{23}.
$$

So the only possible value in the range is 22, but that is even.

...
\mod 23 \mod 23 \mod 23 \mod 23 ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to find an odd integer $t$ with $0 < t < 23$ such that $t + 2$ is the multiplicative inverse of $t$ modulo 23. So the first thing to do is translate that sentence into an equation modulo 23.

If $t + 2$ is the inverse of $t$, then their product should be congruent to 1 modulo 23:

$t(t+2) \equiv 1 \pmod{23}$.

That expands to

$t^2 + 2t - 1 \equiv 0 \pmod{23}$.

Now I can solve this quadratic modulo 23. Formally,

$t = \frac{-2 \pm \sqrt{8}}{2}$.

Since $10^2 \equiv 8 \pmod{23}$, the two solutions are $t = 4$ and $t = 17$.
Among these, only 17 is odd and satisfies the range constraint.
</think>

Therefore the unique odd integer is

$$
\boxed{17}
$$
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The mathematics problem involves solving a modular inverse equation.}

\newpage

%\sampleobs{The four calibration schemes fail in clearly different ways here: the CoT-agnostic Generic-text setting never enters a useful modular reasoning path, the CoT-agnostic Domain-specific setting writes the right equation but closes with the wrong value, and the CoT-aware Stronger-LLM-generated setting misreads the inverse condition. Only the CoT-aware Self-generated setting sustains a complete modular reasoning chain.}

%\samplecase{Right Midpoint, Corrupted Ending}{math-500\_305}

\begin{samplequestion}
If $\frac{\sqrt{2x}}{\sqrt{3x-1}}=\frac32$, solve for $x$. Express your answer in simplest fractional form.
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.33\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
</think>
</think>
Okay, so I need to solve this problem where the ratio of sqrt(2x) over sqrt(3x-1) equals 3/2.

First, let me understand what the problem is asking.
The equation is sqrt(2x)/sqrt(3x-1) = 3/2.

So, maybe I need to think about the ratio as being 2x over 3x-1, but then multiplied by...
Wait, maybe that's not the right way to think about it.

Let me think about the equation again.
Maybe if I square it directly, something simple happens.
Or maybe I should isolate one square root first.

...
Let. Let. Let. Let. Let. Let. ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
To solve the equation
$\frac{\sqrt{2x}}{\sqrt{3x - 1}} = \frac{3}{2}$, we follow these steps.

Step 1: Cross-multiply
$$2\sqrt{2x} = 3\sqrt{3x - 1}$$

Step 2: Square both sides
$$8x = 27x - 9$$

Step 3: Solve
$$x = \frac{9}{19}$$

Step 4: Check the solution
Substituting back gives the correct ratio.

So the solution is 9/19.
Let me write the final answer.

...

The answer is $\boxed{99}$.
The answer is $\boxed{99}$.
[truncated repetitive content]
\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.43\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
I can remove the radicals by squaring, but I should still check the resulting value against the domain and the original equation.

If the algebra stays clean, this should reduce to a single linear equation.
</think>

We are given
$$ \frac{\sqrt{2x}}{\sqrt{3x - 1}} = \frac{3}{2}. $$

Squaring both sides gives
$$ \frac{2x}{3x - 1} = \frac{9}{4}. $$

Cross-multiplying:
$$ 8x = 27x - 9, $$

so
$$ x = \frac{9}{19}. $$
This satisfies the domain condition $x > \frac{1}{3}$.

### Final Answer
$$ \boxed{\frac{9}{19}} $$

...
79
80
81
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to solve

$\frac{\sqrt{2x}}{\sqrt{3x-1}}=\frac{3}{2}$.

The most natural thing is to square both sides, but because square roots are involved I should also check the final result in the original equation.

Squaring gives
$\frac{2x}{3x-1} = \frac{9}{4}$.

Now cross-multiply:
$8x = 27x - 9$.

So $-19x = -9$, hence
$x = \frac{9}{19}$.

Now I should verify it, not just stop there.

Substituting in gives $\frac{\sqrt{18/19}}{\sqrt{8/19}} = \frac{\sqrt{18}}{\sqrt{8}} = \frac{3}{2}$.
</think>

Final Answer:
$$
\boxed{\frac{9}{19}}
$$
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The mathematics problem involves solving a radical equation.}

\newpage

%\sampleobs{Both the CoT-agnostic Domain-specific setting and the CoT-aware Stronger-LLM-generated setting briefly recover the correct intermediate value, but only the CoT-aware Self-generated setting maintains a stable chain through explicit verification and a clean stop.}

\subsection{Coding Reasoning}
\label{code_sample}
% The code cases expose a different failure spectrum. The CoT-agnostic
% Domain-specific and CoT-aware Stronger-LLM-generated settings are often already in
% ``code mode,'' but they may still stop at an unfinished draft, drift into
% over-explanation, or miss one local semantic rule. The CoT-aware
% Self-generated setting is intended to be the cleanest and most complete
% mode, but without looking unrealistically perfect in every intermediate thought
% step.

%\samplecase{Largest Prime Factor: Draft vs. Finished Solver}{humaneval\_plus\_59}

\begin{samplequestion}
def largest_prime_factor(n: int):
    """Return the largest prime factor of n. Assume n > 1 and is not a prime.
    >>> largest_prime_factor(13195)
    29
    >>> largest_prime_factor(2048)
    2
    """
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.33\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
</think>
</think>
</think>
</think>
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
let's think about how to find the largest prime factor of a given number.

One approach is to start by dividing the number by 2 until it's odd.
Then check for odd factors starting from 3 upwards.

Now, let's implement this in code.

def largest_prime_factor(n: int):
    if n % 2 == 0:
        n = n // 2
        while n % 2 == 0:
            n = n // 2
    i = 3
    while i * i <= n:
        while n % i == 0:
            n = n // i
        i += 2
    return n

For n = 13195, the largest prime factor is 239.
[truncated repetitive content]
\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.43\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
I probably want trial division here.
</think>

### Solution Code

def largest_prime_factor(n: int) -> int:
    if n <= 1:
        return -1
    max_prime = 2
    for i in range(2, int(n**0.5) + 1):
        if n % i == 0:
            max_prime = i

At this point I realize the loop is only collecting divisors, not proving primality.
I also have not reduced n while factoring, so this can easily return the wrong thing.

Maybe I should divide by i repeatedly. Or maybe I should check whether i itself is prime first.

Wait, this approach may not be correct.
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to write a function called largest_prime_factor that returns the largest prime factor of n. Since n is guaranteed to be composite and greater than 1, trial division should be enough here.

The main idea is:
1. remove all factors of 2,
2. then scan odd candidates,
3. divide them out when found,
4. keep track of the largest factor I have seen.

I should be careful with powers of 2 and with the case where a large prime factor remains at the end.
</think>

def largest_prime_factor(n: int):
    largest = None
    while n % 2 == 0:
        largest = 2
        n //= 2
    factor = 3
    while factor * factor <= n:
        while n % factor == 0:
            largest = factor
            n //= factor
        factor += 2
    if n > 1:
        largest = n
    return largest
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The coding problem involves finding the largest prime factor.}
\newpage

%\sampleobs{The weaker CoT-agnostic Domain-specific and CoT-aware Stronger-LLM-generated settings are not empty here: both already produce code-like reasoning and implementation. The gap is that the CoT-aware Self-generated setting is the only one that cleanly resolves the factor-versus-prime-factor distinction and finishes the implementation.}

%\samplecase{Uppercase Vowel Counting with a Predicate Bug}{humaneval\_plus\_98}

\begin{samplequestion}
def count_upper(s):
    """
    Given a string s, count the number of uppercase vowels in even indices.
    count_upper('aBCdEf') returns 1
    count_upper('abcdefg') returns 0
    count_upper('dBBE') returns 0
    """
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.21\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
<think>
Okay, I need to implement the function count_upper(s) that counts the number of uppercase vowels in even indices.

First, I need to determine which vowels are considered uppercase.
But in this case, we're looking at uppercase vowels and even indices.
</think>

...
the the the the the the ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
...
So, the function can be implemented as follows:

def count_upper(s):
    count = 0
    vowels = {'A', 'E', 'I', 'O', 'U'}
    for i in range(0, len(s), 2):
        if s[i] in vowels:
            count += 1
    return count

The function correctly counts the number of uppercase vowels in even indices.
\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.32\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
</think>

The task is simple enough that a direct loop over indices should work.

<think>
I only need to check even positions and see whether the character is an uppercase vowel.
But maybe normalizing the character with .upper() will make the condition cleaner.
</think>

def count_upper(s):
    vowels = {'A', 'E', 'I', 'O', 'U'}
    count = 0
    for i in range(len(s)):
        if i % 2 == 0 and s[i].upper() in vowels:
            count += 1
    return count

For example, 'aBCdEf' gives 2.
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to write a function called count_upper that counts uppercase vowels appearing at even indices. This one is short, so the main risk is not the loop but the predicate: it must count only characters that are already uppercase vowels, not lowercase vowels converted to uppercase.

So the clean structure is:
- iterate through even indices only,
- check membership in {'A', 'E', 'I', 'O', 'U'},
- increment the counter.
</think>

def count_upper(s):
    count = 0
    vowels = {'A', 'E', 'I', 'O', 'U'}
    for i in range(0, len(s), 2):
        if s[i] in vowels:
            count += 1
    return count
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The coding problem involves counting uppercase vowels at even indices.}

%\sampleobs{This example keeps the comparison honest: the CoT-agnostic Domain-specific setting can already solve small coding tasks, while the CoT-aware Stronger-LLM-generated setting writes a complete but subtly incorrect predicate by normalizing lowercase vowels before counting them.}

\newpage
%\samplecase{Signed-Digit Semantics Lost in Code Generation}{humaneval\_plus\_108}

\begin{samplequestion}
def count_nums(arr):
    """
    Return the number of elements whose signed digit sum is greater than 0.
    For a negative number, only the first digit is negative:
    e.g., -123 has signed digits -1, 2, and 3.
    """
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.30\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
So, the function is written as follows:
def count_nums(arr):
    "Write a function count_nums ..."

For each element in the array, we need to check if it is a negative number.
If it is, then we need to compute the sum of its digits, but the first digit is negative.

...
the the the the the ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
I need to write a function called count_nums that takes an array of integers and returns the number of elements where the sum of their digits is greater than 0.

Let's implement this in code.


def count_nums(arr):
    count = 0
    for num in arr:
        if num < 0:
            sum_digits = sum(abs(num))
        else:
            sum_digits = sum(abs(num))
        if sum_digits > 0:
            count += 1
    return count

Wait, that would make the sample answer 3, not 1.
\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.45\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
Maybe I should convert each number to a string and handle the negative sign separately.
</think>

<think>
The first signed digit is negative, so the sign only affects the first character after the minus sign. I think I can keep the digits as a string and then reconstruct the sum.
</think>

def count_nums(arr):
    count = 0
    for num in arr:
        s = str(num)
        if s[0] == '-':
            sign = -1
            digits = s[1:]
        else:
            sign = 1
            digits = s
        sum_digits = sum(int(d) for d in digits)
        if sum_digits > 0:
            count += 1
    return count

Wait, but for -123, the signed digits should be -1, 2, 3, so this is still not quite right.
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to count how many numbers have positive signed digit sum. The annoying part is the negative case: for -123, the sum is not -(1+2+3), but rather -1 + 2 + 3.

So I should be careful not to overgeneralize from ordinary digit sums.

One clean way is:
1. turn the absolute value into digits,
2. compute the normal sum,
3. if the original number was negative, subtract twice the first digit to flip only that digit's sign.
</think>

def count_nums(arr):
    count = 0
    for num in arr:
        if num < 0:
            abs_num = abs(num)
            digits = list(map(int, str(abs_num)))
            first_digit = digits[0]
            sum_digits = sum(digits)
            sum_original = sum_digits - 2 * first_digit
        else:
            digits = list(map(int, str(num)))
            sum_original = sum(digits)
        if sum_original > 0:
            count += 1
    return count
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The coding problem involves counting numbers with positive signed digit sum.}

\newpage

%\sampleobs{Both the CoT-agnostic Domain-specific and CoT-aware Stronger-LLM-generated settings are clearly in code-generation mode here, but neither fully internalizes the signed-digit rule. The CoT-aware Self-generated setting is stronger because it reaches the right local semantic correction before writing the final code.}

%\samplecase{Simple Longest-String Task with Long-Tail Self-Justification}{humaneval\_plus\_12}

\begin{samplequestion}
from typing import List, Optional
def longest(strings: List[str]) -> Optional[str]:
    """Return the longest string. Return the first one in case of ties.
    Return None if the input list is empty."""
\end{samplequestion}

\begin{samplegrid}
\setrowheight{0.35\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=genericstrip]{CoT-agnostic: generic-text (C4)}
</think>
Okay, I need to implement the function called "longest strings"
that takes a list of strings and returns the longest one.

The function should return the first one if there are multiple strings
of the same length. If the list is empty, it should return None.

...
So. So. So. So. So. ...
[truncated repetitive content]
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=directstrip]{CoT-agnostic: domain-specific}
I need to implement the function longest(strings: List[str]) -> Optional[str].

The function should return the longest string in the list.
If there are multiple strings of the same maximum length, it should return the first one.
If the list is empty, it should return None.


def longest(strings: List[str]) -> Optional[str]:
    if not strings:
        return None
    max_length = 0
    result = None
    for string in strings:
        if len(string) > max_length:
            max_length = len(string)
            result = string
    return result

The code works for all the cases. The code works for all the cases.
[truncated repetitive content]
\end{samplebox}
\end{samplecol}
\samplegridsep
\setrowheight{0.42\textheight}
\begin{samplecol}
\begin{samplebox}[colbacktitle=strongerstrip]{CoT-aware: stronger-LLM-generated}
<think>
</think>

<think>
This one is just a left-to-right scan with a running best answer.
</think>

from typing import List, Optional

def longest(strings: List[str]) -> Optional[str]:
    if not strings:
        return None
    max_length = 0
    result = None
    for s in strings:
        if len(s) > max_length:
            max_length = len(s)
            result = s
        elif len(s) == max_length:
            pass
    return result

The function handles the edge case of an empty list and returns the first longest string.
\end{samplebox}
\end{samplecol}\samplecolgap
\begin{samplecol}
\begin{samplebox}[colbacktitle=selfstrip]{CoT-aware: self-generated}
<think>
Okay, so I need to write a function called longest that returns the longest string in a list, with the tie-breaking rule that if multiple strings have the same maximum length I keep the first one.

This is actually simple, so I should avoid overthinking it:
- return None if the list is empty,
- scan from left to right,
- only update the answer when I see a strictly longer string.

That way ties automatically keep the earlier string.
</think>

from typing import List, Optional

def longest(strings: List[str]) -> Optional[str]:
    if not strings:
        return None
    max_length = -1
    result = None
    for s in strings:
        if len(s) > max_length:
            max_length = len(s)
            result = s
    return result
\end{samplebox}
\end{samplecol}
\end{samplegrid}
\captionof{figure}{Reasoning examples of 1.58-bit Qwen3-4B models obtained via differentiable ternarization under different calibration schemes. The coding problem involves finding the longest string in a list.}

%\sampleobs{This final example makes the code section more realistic: the CoT-agnostic Domain-specific and CoT-aware Stronger-LLM-generated settings can already solve very simple tasks, but their outputs are still more fragile and more easily polluted by redundant post-hoc explanation than the CoT-aware Self-generated setting.}


==> checklist.tex <==
\newpage
\section*{NeurIPS Paper Checklist}

\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The abstract and introduction contain three parts: i) motivation, ii) methodology, and iii) experimental results, which are explained in Section 1, Section 2, and Section 3.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A \answerNo{} or \answerNA{} answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the limitations in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper has no limitation while the answer \answerNo{} means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate ``Limitations'' section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not include theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer:  \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide all training setups and implementation details in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item If the paper includes experiments, a \answerNo{} answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and\slash or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  The code will be made publicly available. While it is currently under internal review process, we decide not to release the code at this moment.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so \answerNo{} is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://neurips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We detail all experimental settings in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The experiments show consistent and significant improvements over the baseline across multiple model families and evaluation benchmarks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The authors should answer \answerYes{} if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g., negative error rates).
        \item If error bars are reported in tables or plots, the authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide the compute resources in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We have reviewed the NeurIPS Code of Ethics and make sure that our research conforms to it in every respect.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer \answerNo, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification:  We discuss the broader impacts in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that there is no societal impact of the work performed.
        \item If the authors answer \answerNA{} or \answerNo, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate Deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pre-trained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper poses no such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly illustrate the datasets and codebase we use in supplementary materials.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: A set of high-performance 1.58-bit reasoning LLMs are built by the method introduced in this paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset\slash code\slash model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not involve crowdsourcing nor research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The paper does not describe or involve such risks with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does \emph{not} impact the core methodology, scientific rigor, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The development of our core method does not utilize any LLM models.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer \answerNA{} means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy in the NeurIPS handbook for what should or should not be described.
    \end{itemize}

\end{enumerate}
